Generalized Out-of-Distribution Detection: A Survey

Out-of-distribution (OOD) detection is critical to ensuring the reliability and safety of machine learning systems. For instance, in autonomous driving, we would like the driving system to issue an alert and hand over the control to humans when it detects unusual scenes or objects that it has never seen during training time and cannot make a safe decision. The term, OOD detection, first emerged in 2017 and since then has received increasing attention from the research community, leading to a plethora of methods developed, ranging from classification-based to density-based to distance-based ones. Meanwhile, several other problems, including anomaly detection (AD), novelty detection (ND), open set recognition (OSR), and outlier detection (OD), are closely related to OOD detection in terms of motivation and methodology. Despite common goals, these topics develop in isolation, and their subtle differences in definition and problem setting often confuse readers and practitioners. In this survey, we first present a unified framework called generalized OOD detection, which encompasses the five aforementioned problems, i.e., AD, ND, OSR, OOD detection, and OD. Under our framework, these five problems can be seen as special cases or sub-tasks, and are easier to distinguish. We then review each of these five areas by summarizing their recent technical developments, with a special focus on OOD detection methodologies. We conclude this survey with open challenges and potential research directions.

==> sections/4_1_osr.tex <==
\section{Open Set Recognition: Methodology}
\label{sec:osr}
In this section, we introduce the methodology for multi-class ND and open-set recognition (OSR) together. We discuss these two sub-tasks together since both tasks focus on the scenario where ID data comprises multiple classes. The only difference is that OSR has an additional objective to accurately classify the ID data, while multi-class ND produces an ID/OOD binary classifier.% to only retain ID samples and hand them over to standard ID classification.

Since multi-class ND and OSR consider multiple classes during training, most methods are classification-based (Section~\ref{sec:osr_classification}).
Alternative methods are based on ID prototypes (Section~\ref{sec:osr_distance}) and reconstruction  (Section~\ref{sec:osr_reconstruction}).
Few density-based methods will be discussed in Section~\ref{sec:osr_hybrid} along with a discussion. 

\subsection{Classification-based Methods}
\label{sec:osr_classification}
The concept of OSR was first introduced in~\cite{towardosr13pami}, which showed the validity of 1-class SVM and binary SVM for solving the OSR problem. In particular, \cite{towardosr13pami} proposes the 1-vs-Set SVM to manage the open-set risk by solving a two-plane optimization problem instead of the classic half-space of a binary linear classifier. This paper highlighted that the open-set space should also be bounded, in addition to bounding the ID risk.

\subsubsection{EVT-based Uncertainty Calibration}
\label{sec:osr_evt}
Early works observe the overconfidence of neural networks and therefore focus on redistributing the logits by using the compact abating probability (CAP)~\cite{cap14pami} and extreme value theory (EVT)~\cite{evt90appmath,evt12book,psvm14eccv}.
In particular, classic probabilistic models lack the consideration of open-set space. CAP explicitly models the probability of class membership abating from ID points to OOD points, and EVT focuses on modeling the tail distribution with extreme high/low values.
% Building on these two works, W-SVM~\cite{cap14pami} and PI-SVM~\cite{psvm14eccv} trains 1-vs-Set SVM CAP model first and further calibrates the CAP with Weibull distribution, instructed by EVT.
In the context of deep learning, OpenMax~\cite{openmax16cvpr} first implements EVT for neural networks. OpenMax replaces the softmax layer with an OpenMax layer, which calibrates the logits with a per-class EVT probabilistic model such as Weibull distribution.
OpenMax also provides alternative solutions by using penultimate features for EVT modeling, forming a density-based method.
% Taking one step further from simply post hoc calibration of the model uncertainty, techniques such as adversarial training~\cite{advopenmax17bmvc} can be used for improving the quality of deep representations for better performance on the OpenMax layer.

\subsubsection{EVT-Free Confidence Enhancement}
\label{sec:osr_evtfree}
To circumvent the requirement of constructing open-set risks, some works achieved good empirical results without EVT. 
For example, \cite{dtl19cvpr} uses a membership loss to encourage high activations for known classes, and uses large-scale external datasets to learn globally negative filters that can reduce the activations of novel images.
Apart from explicitly forcing discrepancy between known/unknown classes, 
other methods extract stronger features through an auxiliary task of transformation classification~\cite{gdfr20cvpr}, or mutual information maximization between the input image and its latent features~\cite{m2iosr21arxiv}, \etc.

\subsubsection{Unknown Class Generation}
\label{sec:osr_unknownclass}
%The ultimate goal of OSR and multi-label ND is to distinguish between known and unknown samples. 
%Therefore, a straightforward solution is to seek some supervision from unknown samples. 
%Given that the standard OSR and multi-label ND settings do not allow the introduction of unknown samples, 
Image generation techniques have been utilized to synthesize unknown samples from known classes, which helps distinguish between known vs. unknown samples~\cite{gopenmax17bmvc,osrci18eccv,proser21cvpr,kong2021opengan}.
While these methods are promising on simple images such as handwritten characters, they do not scale to complex natural image datasets due to the difficulty in generating high-quality images in high-dimensional space.
Another solution is to successively choose random categories in the training set and treat them as unknown, which helps the classifier to shrink the boundaries and gain the ability to identify unknown classes~\cite{collectdecision20tkde,onevsrest20arxiv}.
Moreover, \cite{intraclass19eusipco} splits the training data into typical and atypical subsets, which also helps learn compact classification boundaries.



\subsection{Distance-based Methods}
\label{sec:osr_distance}
%Comparing to distance-based methods in the one-class scenario in Section~\ref{sec:ad_distance}, their counterparts
Distance-based methods for OSR require the prototypes to be class-conditional, which allows maintaining the ID classification performance.
Category-based clustering and prototyping are performed based on the visual features extracted from the classifiers. OOD samples can be detected by computing the distance \emph{w.r.t.} clusters~\cite{metric18bmvc,podn2020scireport}.
Some methods also leveraged contrastive learning to learn more compact clusters for known classes~\cite{peeler20cvpr,rpl20eccv}, which enlarge the distance between ID and OOD.
CROSR~\cite{crosr19cvpr} enhances the features by concatenating visual embeddings from both the classifier and reconstruction model for distance computation in the extended feature space.
Besides using features from classifiers, GMVAE~\cite{gmvae20aaai} extracts features using a reconstruction VAE, and models the embeddings of the training set as a Gaussian mixture with multiple centroids for the following distance-based operations.
Classifiers using nearest neighbors are also adapted for OSR problem~\cite{nndr17ml}. By storing the training samples, the nearest neighbor distance ratio is used for identifying unknown samples in testing.


\subsection{Reconstruction-based Methods}
\label{sec:osr_reconstruction}
With similar motivations as Section~\ref{sec:ood_reconstruction},
reconstruction-based methods expect different reconstruction behavior for ID vs. OOD samples. The difference can be captured in the latent feature space or the pixel space of reconstructed images. 

\subsubsection{Sparse Representation Methods}
\label{sec:osr_recsparse}
By sparsely encoding images from the known classes, open-set samples can be identified based on their dense representation. Techniques such as sparsity concentration index~\cite{srosr16pami} and kernel null space methods~\cite{knda13cvpr,iknda17cvpr} are used for sparse encoding.

\subsubsection{Reconstruction-Error Methods}
\label{sec:osr_recerror}
By fixing the visual encoder obtained from standard multi-class training to maintain ID classification performance, C2AE trains a decoder conditioned on label vectors and estimates the reconstructed images using EVT to distinguish unknown classes~\cite{c2ae19cvpr}.
Subsequent works use conditional Gaussian distributions by forcing different latent features to approximate class-wise Gaussian models, which enables classifying known samples as well as reject unknown samples~\cite{cgdl20cvpr}.
Other methods generate counterfactual images, which help the model focus more on semantics~\cite{counterfactual21cvpr}.
Adversarial defense is also considered in~\cite{osad20eccv} to enhance model robustness.

\subsection{Discussion}
\label{sec:osr_hybrid}
Although there is not an independent section for density-based methods, these methods can play an important role and are fused as a critical step in some classification-based methods such as OpenMax~\cite{openmax16cvpr}. The density estimation on visual embeddings can effectively detect unknown classes without influencing the classification performance. A hybrid model also uses a flow-based density estimator to detect unknown samples~\cite{openhybrid20eccv}.

Due to the restriction on using only ID data for training, OSR methods do not implement background classes, or outlier exposure (\emph{c.f.} Section~\ref{sec:ood_classification_oe}). A recent research shows that a good classifier~\cite{vaze2021open} in the close-set is comparable to the state-of-the-art OSR methods, which urges the community to develop more general approaches without great efforts on carving for specific datasets.
%However, we believe that background classes-based methods can also benefit OSR settings, as do some other methods from different sub-tasks.

%Recent OOD detection literature encompasses a broader solution space and methodological solutions to detecting the unknowns. 

% \keypoint{Classification Performance}
% \cite{osad20eccv} Open-set Adversarial Defense. First, a decoder is used to ensure that clean images can be reconstructed from the obtained latent features. Then, self-supervision is used to ensure that the latent features are informative enough to carry out an auxiliary task.
% \cite{rdosr20eccv} Representative-Discriminative Learning for Open-set Land Cover Classification of Satellite Imagery.



==> sections/4_2_anomaly.tex <==
\section{Anomaly Detection \& Novelty Detection: Methodology}
\label{sec:anomaly}
In this section, we review methodologies for AD and one-class ND. 
Most of the methods for sensory AD and semantic AD are shared, except for sensory AD focuses more on local information in the images and internal information of neural networks.\@
Moreover, semantic AD and one-class ND have the same problem formulation (recall Section~\ref{sec:tax_novelty}), therefore we review the methods for these three sub-tasks altogether.

Given the homogeneous in-distribution data, a straightforward approach is to estimate the in-distribution density and reject OOD test samples that deviate from the estimated distribution. We summarize density-based methods in Section~\ref{sec:ad_density}.
Alternative methods rely on the quality of image reconstruction to distinguish anomalous samples (Section~\ref{sec:ad_reconstruction}), or directly learn a decision boundary between ID and OOD data
 (Section~\ref{sec:ad_classification}). We also review 
distance-based in Section~\ref{sec:ad_distance}.
Lastly, we conclude with a discussion and present theoretical works in Section~\ref{sec:ad_hybrid}.

\subsection{Density-based Methods}
\label{sec:ad_density}
Density-based methods attempt to model the distribution of normal data (ID),
with an operating assumption that anomalous test data has low likelihood whereas normal data has higher likelihood under the estimated density model. 

\subsubsection{Classic Density Estimation}
\label{sec:ad_density_classic}
\keypoint{a.~Parametric Density Estimation}
Parametric density estimation assumes the ID density can be expressed through some pre-defined distributions~\cite{anomalyparametric98pami}.
One approach is to fits a multivariate Gaussian distribution on the training data and measures the Mahalanobis distance between the test sample and the expectation of training samples~\cite{mahalanobis00cils,mahalanobis18jesp}.
Other works adopt more complex assumptions on in-distribution, such as mixed Gaussian distribution~\cite{gmm84siam,anomalygmm00icml}, and Poisson distribution~\cite{poisson16isi}, \etc.

\keypoint{b.~Non-parametric Density Estimation}
Nonparametric density estimation solves a more practical scenario where a predefined distribution is unable to model the real distribution~\cite{nonparametric91jasa}.
One can simply model the training distribution with histograms~\cite{histogram73cstm,histogram12wireless,histogram09traffic,hbos12ki}.
Kernel density estimation (KDE) further uses the kernel function as a continuous replacement for the discrete histogram~\cite{kde62math,kdeanomaly98ime,anomalykde18tkde}. 
It flexibly takes parameters such as point weights and bandwidth to control the estimated distribution.

\keypoint{Discussion}
Although the classic density estimation methods obtain strong AD performance on wide ranges of tasks~\cite{adpower82iee,admisuse93tse}, they are better suited for low-dimensional data.
For high-dimensional data in computer vision tasks, these methods suffer from computational and scalability issues due to the curse of dimensionality~\cite{adhighdim20jcgs}.
To alleviate the problem, shallow methods implement feature engineering to reduce the dimensionality~\cite{adoverview07cn,adcrowdedscene10cvpr}.

\subsubsection{Density Estimation with Deep Generative Models}
\label{sec:ad_density_nn}
In the context of deep learning, neural networks can produce features with high representation quality, which significantly enhance the performance of classic density estimation.

\keypoint{a.~AE/VAE-based Models}
An autoencoder~(AE) learns efficient representations of unlabeled data by reconstructing the input from the latent embedding~\cite{ae91aiche}. Variational autoencoder~(VAE)~\cite{vae13arxiv} encodes input images into latent vectors under the Gaussian distribution.
The learned encoding can be considered as the lower-dimensional representation of the input.
Classic density estimation methods can then be applied on top of these deep representations~\cite{dagmm18iclr,autogres19cvpr,gpnd18nips}.


\keypoint{b.~GAN-based Models}
Generative adversarial networks (GANs) consist of a generative network and a discriminative network,  contesting with each other in a zero-sum game~\cite{gan14nips}. 
Typically, the generative network learns to map from a latent space to a data distribution of interest, whereas the discriminative network distinguishes candidates produced by the generator from the true data distribution.
However, unlike the previous AE/VAE paradigm, the lack of an encoder makes it difficult for a GAN to directly find the corresponding embedding for a given image.
To solve the problem, ADGAN~\cite{adgan18ecml} searches for a good representation in the latent space for a given sample. If such a representation is not found, the sample is deemed anomalous. However, this method can be computationally expensive.

\keypoint{c.~Flow-based Models}
A normalizing flow describes the transformation of a probability density through a sequence of invertible mappings. By repeatedly applying the rule for change of variables, the initial density ``flows'' through the sequence of invertible mappings~\cite{flows15icml,flowreview20pami}.
Therefore, methods with the normalizing flow can directly estimate the likelihood of the input space.
The flow-based methods are appraised by their elegant mathematical presentations, and are also shown to be sensitive to low-level features only.  Flow-based methods can lead to significant computational costs since no dimensionality reduction is performed.

\keypoint{d.~Representation Enhancement}
Apart from obtaining visual embeddings through generative models, some methods focus on enhancing the model capacity to increase the representation power of the extracted features, which may better characterize the normality/ID-ness for more accurate density estimation.
These strategies include data augmentation~\cite{cutpaste21cvpr}, adversarial training~\cite{gpnd18nips}, distillations~\cite{distill21cvpr}, loss function enhancement~\cite{losscalad18nips}, and usage of shallow~\cite{multiatt21cvpr,mlloo20aaai} and local features~\cite{localae20cikm}.

\subsubsection{Energy-based Models}
\label{sec:ad_energy}
Energy-based model (EBM) is a generative model that uses a scalar energy score to express the probability density of variables through unnormalized negative log probability~\cite{energy11icml},
which provides a valid solution for AD~\cite{energyad16icml}.
However, compared to standard deep learning models, the training process of EBMs can be computationally expensive, since MCMC sampling and approximations are required to calculate integrals.
To address the problem, methods such as the score matching method~\cite{scorematch05jmlr} and stochastic gradient Langevin dynamics~\cite{sgld11icml} are proposed for efficient training. 

\subsubsection{Frequency-based Methods}
\label{sec:ad_frequency}
Previous works also explored frequency domain analysis for anomaly detection. 
While humans perceive images based on low-frequency components, CNN models can largely depend on high-frequency components for decision-making~\cite{highfreq20cvpr,adversarialbugs19nips}.
Methods such as CNN kernel smoothing~\cite{highfreq20cvpr} and spectrum-oriented data augmentation~\cite{amplitude21iccv} are proposed to suppress the influence of high-frequency components.
Other works also find that adversarial attacks on low-frequency components are also difficult to detect, therefore proposing methods to target the phase spectrum~\cite{phase21cvpr}.
Frequency-based methods mainly focus on sensory AD (especially on detecting adversarial examples).

\subsection{Reconstruction-based Methods}
\label{sec:ad_reconstruction}
Similar to Section~\ref{sec:osr_reconstruction}, some AD methods rely on the different performance on performing normal and abnormal data to identify anomalies. 
The difference of model performance can be measured in the feature space (Section~\ref{sec:ad_recsparse}) or by the reconstruction error (Section~\ref{sec:ad_reconstructionerror}).
%For example, the feature sparsity can be used as an anomaly indicator, which we describe in Section~\ref{sec:ad_recsparse}. We will also describe the reconstruction-based methods in Section~\ref{sec:ad_reconstructionerror}, where ID data is expected to have a smaller reconstruction error than that of OOD counterparts. 
% For reconstructed outputs, the expected observation of better quality of ID reconstruction over OOD counterparts yields the reconstruction-error method, to be introduced in Section~\ref{sec:ad_reconstructionerror}.

\subsubsection{Sparse Representation}
\label{sec:ad_recsparse}
Sparse reconstruction assumes that every normal sample can be reconstructed accurately using a limited set of basis functions, whereas anomalous data should suffer from larger reconstruction costs, thus generating a dense representation~\cite{admm15jsps,adsparsecrowd17mta,adsparsevideo13tcsvt}. Exemplar techniques for sparse encoding include $L_1$ norm-based kernel PCA~\cite{kpca13pr} and low-rank embedded networks~\cite{lren21aaai}.

\subsubsection{Reconstruction-Error Methods}
\label{sec:ad_reconstructionerror}
Reconstruction-error methods rely on the assumption that a reconstruction model trained on the normal data will produce higher-quality outcomes for normal test samples as opposed to anomalies. 
Deep reconstruction models include AEs~\cite{recerrae18wts}, VAEs~\cite{recerrvae15ie}, GANs~\cite{ganad18iclr}, and U-Net~\cite{framepred18cvpr} that can all be used as the backbone for this method.

\keypoint{a.~AE/VAE-based Models}
Apart from the standard combination of reconstruction-error and AE/VAE models~\cite{recerrae18wts,recerrvae15ie},
other methods use more sophisticated strategies such as reconstructing by memorized normality~\cite{menae19iccv,memad20cvpr}, adapting model architectures~\cite{rsr20iclr}, and partial/conditional reconstruction~\cite{scadn21aaai,gpnd18nips,conad19icml}.
In the semi-supervised AD setting, CoRA~\cite{cora19aaai} trains two AEs on inliers and outliers respectively. The reconstruction errors derived from the two AEs can be used as an indicator of anomaly. 

\keypoint{b.~GAN-based Models}
Advancement in generative modeling has led to the remarkable development of reconstruction-error methods using GANs.
The discriminator in GANs intrinsically calculates the reconstruction error for anomaly detection~\cite{ganad18iclr}.
Moreover, variants of GANs---such as denoising GANs~\cite{advrec18cvpr} and class-conditional GANs~\cite{ocgan19cvpr}---enable further performance improvement by increasing the reconstruction difficulty.
Some methods utilize the performance of the reconstructed image in downstream tasks to further amplify the reconstruction error of anomalies~\cite{pnet20eccv}.
Ensembling can also enhance the performance~\cite{ganesb21aaai}.


\subsubsection{Gradient-based Methods}
\label{sec:ad_recmeta}
Gradient-based method belongs to meta-learning or learning to learn, which is a topic of systematically observing the internal mechanisms of the learning tasks or models to propose methods based on the learned experience, or meta-data~\cite{metalearningsurvey18arxiv,metalearningsurvey20arxiv}.
To address AD tasks, some method observes the different patterns on training gradient between normalities and anomalies in a reconstruction task and hence use gradient-based representation to characterize anomalies~\cite{gradcon20eccv}.


\subsection{Distance-based Methods}
\label{sec:ad_distance}
Distance-based methods detect anomalies by calculating the distance between targeted samples and a number of internally stored exemplars, or prototypes~\cite{wettschereck1994study}.
These methods usually require training data in the memory. Representative methods include K-nearest Neighbors~\cite{tian2014anomaly}, prototype-based methods~\cite{munz2007traffic,syarif2012unsupervised}, as well as methods to be introduced in Section~\ref{sec:od_distance}.

%, and can therefore be interpreted as outlier detection methods



\subsection{Classification-based Methods}
\label{sec:ad_classification}
AD and one-class ND is often formulated as an unsupervised learning problem,
where the entire ID data belongs to one class. Fully supervised AD is studied in~\cite{supervisedad13jair}. %While classification-based methods seem incompatible, 
%, except for some minor fully supervised AD tasks~\cite{supervisedad13jair}.
The idea of classifier boundaries is successfully implemented and marked as a one-class classification task~\cite{occ02tax,occsurvey09icaics}, which we describe in Section~\ref{sec:ad_occ}.
When it comes to semi-supervised AD setting where unlabeled data is introduced for training, PU learning is proposed for this specific problem,
which will be introduced in Section~\ref{sec:ad_pulearing}.
Lastly, we introduce self-supervised learning methods in Section~\ref{sec:ad_ssl}.% can further enhance the feature quality for generally better AD performance. Alternatively, the performance of a well-designed surrogate task can reveal the anomalies eventually.

\subsubsection{One-Class Classification}
\label{sec:ad_occ}
One-class classification (OCC) directly learns a decision boundary that corresponds to a desired density level set of the normal data distribution~\cite{occ02tax}.
DeepSVDD~\cite{deepsvdd18icml} first introduced the classic OCC to the deep learning community, which maps normal/ID examples into a hypersphere so that the description of normality is bounded. Deviations from this description are then deemed to be anomalies.
Later, some works try to extend the method through elastic regularization~\cite{panda21cvpr} or constructing an adapted description with multi-linear hyperplanes~\cite{gods19iccv}.

\subsubsection{Positive-Unlabeled Learning}
\label{sec:ad_pulearing}
Positive-unlabeled learning, or PU learning, focuses on the semi-supervised AD setting where unlabeled data is available in addition to the normal data~\cite{pusurvey08isip,pusurvey20ml,pusurvey19iisa,deepsad20iclr}.
The unlabeled data can contain both positive and negative examples.
Popular PU learning methods generally rely on two strategies.
One approach is to select reliable negative samples from unlabeled data and convert them into the supervised AD setting. Techniques such as distance to prototypes~\cite{psol06bioinfo,rocchio03ijcai,pulearnknn09jcomp}, clustering~\cite{pulearncluster12iconip,pulearncluster14jise}, and density-based models~\cite{bayesianrelabel18arxiv} are used to filter out reliable negatives.
Others consider the entire unlabeled set as noisy negatives, converting it into learning with noisy labels setting. Techniques such as sample re-weighting~\cite{puleanclassest15icml} and label cleaning methods~\cite{pulearnmixture15ais,gcnclean19cvpr} have also shown their effectiveness for the task.
Besides, reconstruction-error methods can be re-purposed for PU learning by training two reconstruction models for the positive and unlabeled set, respectively~\cite{comprec19aaai}. The comparison between their reconstruction-error scores indicates the final AD decision.

\subsubsection{Self-Supervised Learning}
\label{sec:ad_ssl}
Self-supervised learning methods tackle the AD and one-class ND problems in two aspects: (1) the enhancement of feature quality can improve AD performance; (2) some well-designed surrogate tasks can help reveal the anomalies from normal samples.
In this part, we only discuss the second pretext task designing, since the first methods that improve feature quality are introduced with their corresponding main tasks, such as in Section~\ref{sec:ad_density_nn}.
One classic method is isolation forest~\cite{isoforest08icdm}, which generates a random forest to contrast every normal sample. A test anomaly can be isolated in fewer steps than normal instances.
Other methods use pretext tasks such as contrastive learning~\cite{csi20nips} and image transformation prediction~\cite{goad20iclr,transform18nips}, where anomalies are more likely to make mistakes on the designed task. For video data, a natural self-supervised task is to predict future frames based on the existing ones~\cite{ssmtl21cvpr}, where larger error indicates abnormalities.


\subsection{Discussion}
\label{sec:ad_hybrid}

\keypoint{Sensory \vs.~Semantic AD} 
%Even with the different definitions of anomalies, 
Sensory and semantic AD both consider the normality as homogeneous, even though there might be multiple categories in the normal data. Solutions to semantic AD are mostly applicable to sensory AD problems. In particular, sensory AD problems can benefit from methods that focus on lower-level features (\eg flow-based and hidden feature-based), local representations, and frequency-based methods (\cf Section~\ref{sec:ad_frequency}).


\keypoint{Theoretical Analysis}
In addition to algorithmic development, several works provided theoretical analysis on AD and one-class ND.
In \cite{pac18icml}, a clean set of ID and a mixed set of ID/OOD are constructed with identical sample sizes. 
A PAC-style finite sample guarantee is achieved for a certain probability of detecting a certain portion of anomalies with the minimum number of false alarms.
Furthermore, in~\cite{bound21icml}, a generalization error bound is provided for PU learning methods in semi-supervised AD. 

\keypoint{Anomaly Detection \vs. Outlier Detection}
If we model the test samples and training samples altogether, the AD problem will be transformed into an OD problem, and therefore the transductive approaches in Section~\ref{sec:outlier} are also applicable. However, this method requires all training data to estimate test abnormality, which greatly increases the storage burden and computational complexity. Therefore, we do not include these methods in this part, but leave it to Section~\ref{sec:outlier}. 

==> sections/4_3_outlier.tex <==
\section{Outlier Detection: Methodology}
\label{sec:outlier}
Outlier detection (OD) requires the observation of all samples and aims to detect those that deviate significantly from the majority distribution. OD approaches are usually transductive, rather than inductive. Several surveys reviewed methodologies on this topic, yet mostly within the field of data mining~\cite{outlierhighd01sigmod,outliersurvey04aireview,outlier05handbook,outlierprogress19ieee}. In this section, we briefly review OD methods, especially those developed for computer vision tasks using deep neural networks. 
We find that although deep learning methods rarely directly solve the OD problem, the data cleaning procedure, which is the prerequisite procedure of learning from open-set noisy data~\cite{iterativeosnl18cvpr,webly15iccv} and open set semi-supervised learning~\cite{openworldssl21arxiv}, are solving the OD tasks.

\subsection{Density-based Methods}
\label{sec:od_density}
A basic idea of OD models the entire dataset as a Gaussian distribution and flags samples that are at least three standard deviations from the mean~\cite{std05bmj,devmedian13jesp}. Other parametric probabilistic methods make use of Mahalanobis distance~\cite{mahalanobis00cils} and Gaussian mixtures~\cite{gmm09siam} to model the data density.
Similar to the ``three standard deviations'' rules, the interquartile range can also be used to identify outliers~\cite{ir14bmc}, forming a classic non-parametric probabilistic method.
Local outlier factor (LOF) estimate the density of a given point via the ratio of the local reachability of its neighbors and itself~\cite{lof00sigmod}, 
followed by derivations for robustification~\cite{cof02pakdd,loop09ikm} and simplification~\cite{simplelof14dmkd}.
RANSAC~\cite{fischler1981random} iteratively estimates parameters of a mathematical model to fit the data and find the samples as outliers that contribute less to estimates.
Generally, classic density methods for AD such as kernel density estimation (\cf Section~\ref{sec:ad_density}) are also applicable for OD.
Although these methods suffer from the curse of dimensionality on images, they can be alleviated by dimensionality reduction methods~\cite{pcaoutlier11dmkd,matsket18nips} and the NN-based density methods~(\cf Section~\ref{sec:ad_density}).

\subsection{Distance-based Methods}
\label{sec:od_distance}
A simple method to detect outliers is counting the number of neighbors within a certain radius, or measure the $k$th-nearest neighbor distance~\cite{distanceod13nips,distanceod10vldb}. %The effects of distance are also reflected by LOF in the previous part.
We mainly discuss cluster-based methods and graph-based methods here.

\subsubsection{Cluster-based Methods}
\label{sec:od_cluster}
DBSCAN~\cite{dbscan96kdd} accumulates samples based on the distance-based density to form clusters. Samples that lie outside the major clusters are recognized as outliers. Subsequent works improve the clustering approaches by considering the confidence of cluster labels~\cite{clusterod07ecml}.

\subsubsection{Graph-based Methods}
\label{sec:od_graph}
Another set of methods uses the relationship among data points and constructs a neighborhood graph~\cite{knngraph04icpr,neibourgraph04jiis} or its variants~\cite{largegraph10icml}. Graph properties and graph mining techniques are employed to find abnormal samples~\cite{graphad15dmkd,graphad03sigkdd}, such as graph-based clustering~\cite{gbc07ictai,gbc12iccse}, partitioning~\cite{ngc21iccv}, and label propagation with graph neural networks~\cite{webly20acmmm}.

\subsection{Classification-based Methods}
\label{sec:od_classification}
 AD methods (\eg Isolation Forest~\cite{isoforest08icdm}, OC-SVM~\cite{occ02tax,deepsvdd18icml}, \etc) are also applicable to OD setting. When there are multiple classes in the dataset, researchers find that deep learning models---when trained with outliers---can still show robust prediction capability and identify the outliers~\cite{li2017learning}. Data cleaning using large pre-trained models is also common in the industry.
Techniques to enhance model robustness and feature generalizability can be useful for this task, such as ensembling~\cite{nguyen2019self}, co-training~\cite{han2018co}, and distillation~\cite{li2017learning,webly20eccv}.

\subsection{Discussion}
Although the application of OD is not as common as other sub-tasks in the computer vision community, techniques for OD can be valuable for other tasks such as open-set semi-supervised learning, learning with open-set noisy labels, and potentially novelty discovery.
In addition to methods reviewed here, most solutions to AD/ND/OOD detection can also be applied by considering all observations as ID (for model training) and then applying the model again on all the observations. In this case, methods such as reconstruction-based PCA (\cf Section~\ref{sec:ad_reconstruction}) and energy-based models (\cf Section~\ref{sec:ad_energy} and \ref{sec:ood_confcal}) can also address the OD problem.




==> sections/paper_list_old.tex <==
\begin{table*}[]
\caption{Paper list for generalized out-of-distribution detection tasks.}
\label{tab:method}
\centering
\begin{tabular}{@{}c|c|l|p{8cm}<{\centering}@{}}
\toprule
Task & \multicolumn{2}{c|}{Methodology} & Reference \\ \midrule
\midrule
\multirow{15}{*}{\begin{tabular}[c]{@{}c@{}}\textcolor{red}{$\S$}~\ref{sec:ood}\\ Out-of-Distribution \\ Detection\end{tabular}} &
\multicolumn{1}{c|}{\multirow{11}{*}{\begin{tabular}[c]{@{}c@{}} \textcolor{red}{$\S~$}\ref{sec:ood_classification} \\ Classification \end{tabular}}} & \textcolor{red}{$\S~$\ref{sec:ood_confcal}.a}:~Post-hoc Detection  
& \cite{msp17iclr,odin18iclr,energyood20nips, wang2021canmulti, sun2021tone, huang2021importance, gram20icml} \\  \cmidrule(l){3-4} 
& \multicolumn{1}{c|}{}                                     & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} \textcolor{red}{$\S~$\ref{sec:ood_confcal}.b}:~Conf. Enhancement \end{tabular}}
& \cite{confbranch2018arxiv,wang2021energy,ceda19cvpr,eloc18eccv,good20nips,aloe20arxiv,whyrelu19cvpr,blur20iclr,mixup19nips,cutmix19cvpr,cutout17arxiv,augmix19arxiv,ccu20arxiv,mood21cvpr,mahananobis18nips,gram20icml,gram19nipsw,gram20cvprw,godin20cvpr} \\ \cmidrule(l){3-4} \cmidrule(l){3-4}
& \multicolumn{1}{c|}{}                                     & \textcolor{red}{$\S~$\ref{sec:ood_classification_oe}.c}:~Outlier Exposure (OE)         
& \cite{oe18nips,agnostophobia18nips,mcd19iccv,oecc21neurocomputing,backgroundsampling20cvpr,outliermining21ecml,pseudolabel20aaai,yang2021scood,abstention21arxiv,lessbias19bmvc, sina2020aaai} \\ \cmidrule(l){3-4} 
& \multicolumn{1}{c|}{}                                     & \textcolor{red}{$\S~$}\ref{sec:ood_classification_oegen}:~OOD Data Generation             & \cite{confcal18iclr,oodsg19nipsw,confgan18nipsw,zsar19cvpr}          \\  \cmidrule(l){3-4} 
& \multicolumn{1}{c|}{}                                     & \textcolor{red}{$\S~$}\ref{sec:ood_gradient}:~Gradient-based Methods             & \cite{odin18iclr,huang2021importance}          \\
\cmidrule(l){3-4} 
& \multicolumn{1}{c|}{}                                     & \textcolor{red}{$\S~$\ref{sec:ood_bayesian}}:~Bayesian Models         
& \cite{mcdropout16icml,deepensemble17nips,practicalbnn19nips,dpn18nips,dpn19nips,dpn20nips} \\
\cmidrule(l){3-4} 
& \multicolumn{1}{c|}{}                                     & \textcolor{red}{$\S~$}\ref{sec:ood_pretrain}:~Large-scale OOD Detection  & \cite{nearood21arxiv,pretransformer20arxiv,oodformer21arxiv, mos21cvpr} \\
\cmidrule(l){2-4} 
& \multicolumn{2}{c|}{
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
\textcolor{red}{$\S~$}\ref{sec:ood_density}:~Density-based Methods
\end{tabular}}}
% & \multicolumn{1}{c|}{\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} \textcolor{red}{$\S~$}\ref{sec:ood_density}\\Density\end{tabular}}}             
% & \multicolumn{1}{l|}{\multirow{2}{*}{\textcolor{red}{$\S~$}\ref{sec:ood_density_nn}:~Density Estimation}}     
& \cite{dagmm18iclr,autogres19cvpr,gpnd18nips,adgan18ecml,advrec18cvpr,mahananobis18nips,flowreview20pami,residualflow20cvpr,glow18nips,pixelcnn16icml,dgmknow19nips,waic18arxiv,whyflow20nips,likelihoodratio19nips,ratiogm20iclr,vae20nips} \\ 
% \cmidrule(l){3-4} 
% & \multicolumn{1}{c|}{}                                     & \textcolor{red}{$\S~$}\ref{sec:ood_energy}:~Energy-based Models             & \cite{scorematch05jmlr,sgld11icml,secretebm20iclr,energyood20nips} \\ 
\cmidrule(l){2-4} 
& \multicolumn{2}{c|}{\textcolor{red}{$\S~$}\ref{sec:ood_distance}:~Distance-based Methods}               & \cite{mahananobis18nips,rmd21arxiv,cosinesim20accv,svae20eccv,onedim21cvpr,duq20icml,fss20arxiv} \\ 
\midrule
\midrule
\multirow{10}{*}{\begin{tabular}[c]{@{}c@{}}\textcolor{red}{$\S$}~\ref{sec:osr}\\ Open Set \\ Recognition\end{tabular}} &
\multicolumn{1}{c|}{\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}} \textcolor{red}{$\S~$}\ref{sec:osr_classification}\\Classification\end{tabular}}} & \textcolor{red}{$\S~$}\ref{sec:osr_evt}:~EVT-based Calibration &
\cite{cap14pami,psvm14eccv,openmax16cvpr,advopenmax17bmvc} \\ \cmidrule(l){3-4} 
& \multicolumn{1}{c|}{}                                     & \textcolor{red}{$\S~$}\ref{sec:osr_evtfree}:~EVT-free Calibration & \cite{dtl19cvpr,gdfr20cvpr,m2iosr21arxiv} \\ \cmidrule(l){3-4} 
& \multicolumn{1}{c|}{}                                     & \textcolor{red}{$\S~$}\ref{sec:osr_unknownclass}:~Unknown Generation & \cite{gopenmax17bmvc,osrci18eccv,proser21cvpr,kong2021opengan,collectdecision20tkde,onevsrest20arxiv,intraclass19eusipco} \\
\cmidrule(l){3-4} 
& \multicolumn{1}{c|}{}                                     & \textcolor{red}{$\S~$}\ref{sec:osr_labelspace}:~Label Space Redesign & \cite{hierarchical18cvpr,mos21cvpr,ksemantic18nips,clip21arxiv,nearood21arxiv,gan2021language} \\
\cmidrule(l){2-4} 
& \multicolumn{2}{c|}{\textcolor{red}{$\S~$}\ref{sec:osr_distance}:~Distance-based Methods}                & \cite{metric18bmvc,podn2020scireport,peeler20cvpr,rpl20eccv,crosr19cvpr,gmvae20aaai,nndr17ml} \\ \cmidrule(l){2-4} 
& \multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}} \textcolor{red}{$\S~$}\ref{sec:osr_reconstruction}\\Reconstruction\end{tabular}}}      & \textcolor{red}{$\S~$}\ref{sec:osr_recsparse}:~Sparse Representation    &
\cite{srosr16pami,knda13cvpr,iknda17cvpr} \\ \cmidrule(l){3-4} 
& \multicolumn{1}{c|}{}                                     & \textcolor{red}{$\S~$}\ref{sec:osr_recerror}:~Reconstruction-Error & 
\cite{c2ae19cvpr,cgdl20cvpr,counterfactual21cvpr,osad20eccv} \\ 
\midrule
\midrule
\multirow{19}{*}{\begin{tabular}[c]{@{}c@{}} \textcolor{red}{$\S$}~\ref{sec:anomaly}\\ Anomaly Detection \\\& \\ Novelty Detection \end{tabular}} &
\multicolumn{1}{c|}{\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}} \textcolor{red}{$\S~$}\ref{sec:ad_density}\\Density\end{tabular}}}  & \textcolor{red}{$\S~$}\ref{sec:ad_density_classic}:~Classic Density Est. 
& \cite{anomalyparametric98pami,mahalanobis18jesp,anomalygmm00icml,poisson16isi,nonparametric91jasa,anomalykde18tkde} \\ 
\cmidrule(l){3-4}
& \multicolumn{1}{c|}{}                 &
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} \textcolor{red}{$\S~$}\ref{sec:ad_density_nn}:~NN-based Density Est. \end{tabular}}
% \textcolor{red}{$\S~$}\ref{sec:ad_density_nn}:~NN-based Density Est.
& \cite{dagmm18iclr,autogres19cvpr,gpnd18nips,adgan18ecml,flows15icml,flowreview20pami,cutpaste21cvpr,gpnd18nips,distill21cvpr,losscalad18nips,multiatt21cvpr,mlloo20aaai,localae20cikm}
\\ \cmidrule(l){3-4} 
& \multicolumn{1}{c|}{}                 & \textcolor{red}{$\S~$}\ref{sec:ad_energy}:~Energy-based Models        & \cite{energyad16icml,scorematch05jmlr,sgld11icml} \\ 
\cmidrule(l){3-4} 
& \multicolumn{1}{c|}{}                 & \textcolor{red}{$\S~$}\ref{sec:ad_frequency}:~Frequency-based Methods        & \cite{highfreq20cvpr,adversarialbugs19nips,amplitude21iccv,phase21cvpr} \\ 
\cmidrule(l){2-4} 

& \multicolumn{1}{c|}{\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} \textcolor{red}{$\S~$}\ref{sec:ad_reconstruction}\\Reconstruction\end{tabular}}}      & \textcolor{red}{$\S~$}\ref{sec:ad_recsparse}:~Sparse Representation    &
\cite{admm15jsps,adsparsecrowd17mta,adsparsevideo13tcsvt,kpca13pr,lren21aaai} \\ \cmidrule(l){3-4} 
& \multicolumn{1}{c|}{}                                     & 
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} \textcolor{red}{$\S~$}\ref{sec:ad_reconstructionerror}:~Reconstruction-Error \end{tabular}} & 
\cite{recerrae18wts,recerrvae15ie,ganad18iclr,framepred18cvpr,recerrae18wts,recerrvae15ie,menae19iccv,memad20cvpr,rsr20iclr,scadn21aaai,gpnd18nips,conad19icml,cora19aaai,ganad18iclr,advrec18cvpr,ocgan19cvpr,pnet20eccv,ganesb21aaai}
\\ \cmidrule(l){2-4} 
& \multicolumn{1}{c|}{\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}} \textcolor{red}{$\S~$}\ref{sec:ad_classification}\\Classification\end{tabular}}} & \textcolor{red}{$\S~$}\ref{sec:ad_occ}:~One-Class Classification &
\cite{occ02tax,deepsvdd18icml,panda21cvpr,gods19iccv} \\ \cmidrule(l){3-4} 
& \multicolumn{1}{c|}{}                                     &  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} \textcolor{red}{$\S~$}\ref{sec:ad_pulearing}:~PU Learning  \end{tabular}} & 
\cite{pusurvey08isip,pusurvey20ml,pusurvey19iisa,psol06bioinfo,rocchio03ijcai,pulearnknn09jcomp,pulearncluster12iconip,pulearncluster14jise,bayesianrelabel18arxiv,puleanclassest15icml,pulearnmixture15ais,gcnclean19cvpr,comprec19aaai}
\\ \cmidrule(l){3-4} 
& \multicolumn{1}{c|}{}                                     & \textcolor{red}{$\S~$}\ref{sec:ad_ssl}:~Self-Supervised Learning  & \cite{isoforest08icdm,csi20nips,goad20iclr,transform18nips,ssmtl21cvpr}
\\ \cmidrule(l){2-4} 
& \multicolumn{2}{c|}{\textcolor{red}{$\S~$}\ref{sec:ad_distance}:~Distance-based Methods}
& \cite{tian2014anomaly,munz2007traffic,syarif2012unsupervised} \\ \cmidrule(l){2-4} 
& \multicolumn{2}{c|}{\textcolor{red}{$\S~$}\ref{sec:ad_meta}:~Gradient-based Methods}          & \cite{gradcon20eccv} \\ \cmidrule(l){2-4} 
& \multicolumn{2}{c|}{\textcolor{red}{$\S~$}\ref{sec:ad_hybrid}:~Discussion and Theoretical Analysis}                 & \cite{pac18icml,bound21icml} \\
\midrule
\midrule
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}\textcolor{red}{$\S$}~\ref{sec:outlier}\\ Outlier \\ Detection\end{tabular}} &
\multicolumn{2}{c|}{ \textcolor{red}{$\S~$}\ref{sec:od_density}:~Density-based Methods}
& \cite{ir14bmc,lof00sigmod,cof02pakdd,loop09ikm,simplelof14dmkd,fischler1981random,pcaoutlier11dmkd,matsket18nips} \\
\cmidrule(l){2-4} 
& \multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}} \textcolor{red}{$\S~$}\ref{sec:od_distance}\\Distance\end{tabular}}}             
& \multicolumn{1}{l|}{\textcolor{red}{$\S~$}\ref{sec:od_cluster}:~Cluster-based Methods}  
& \cite{dbscan96kdd,clusterod07ecml} \\ \cmidrule(l){3-4} 
& \multicolumn{1}{c|}{}                                     & \textcolor{red}{$\S~$}\ref{sec:od_graph}:~Graph-based Methods  & \cite{graphad15dmkd,graphad03sigkdd,gbc07ictai,gbc12iccse,webly20acmmm} \\ \cmidrule(l){2-4} 
& \multicolumn{2}{c|}{$\S~$\ref{sec:od_classification}:~Classification-based Methods} & \cite{isoforest08icdm,occ02tax,deepsvdd18icml,li2017learning,nguyen2019self,han2018co,webly20eccv} \\
\bottomrule
\end{tabular}
\end{table*}
